Formal Model Guided Conformance Testing for Blockchains

Modern blockchains increasingly consist of multiple clients that implement a single blockchain protocol. If there is a semantic mismatch between the protocol implementations, the blockchain can permanently split and introduce new attack vectors. Current ad-hoc test suites for client implementations are not sufficient to ensure a high degree of protocol conformance. As an alternative, we present a framework that performs protocol conformance testing using a formal model of the protocol and an implementation running inside a deterministic blockchain simulator. Our framework consists of two complementary workflows that use the components as trace generators and checkers. Our insight is that both workflows are needed to detect all types of violations. We have applied and demonstrated the utility of our framework on an industrial strength consensus protocol.

==> applications.tex <==
\section{Other Applications}
\label{sec:app}
In this section we describe other applications that be performed with our framework in conjunction with conformance testing. 


\paragraph{\bf Performance Conformance}
Thus far, we have discussed semantic conformance. However, in blockchains, there are often performance requirements that new
clients need to adhere to. For example, these could be measured in metrics such as time to finality (TTF), transactions per second (TPS) or even more nuance metrics measuring internal aspects of a particular protocol. Our deterministic simulator is instrumented to measure base metrics such as time, number of transactions, number of vertices, etc. Users can configure the simulator to produce derived metrics and plot the metrics against each other. This allows users to fuzz or specify a particular scenario to see how the protocol under test performs. 

\paragraph{ \bf Diagnostics, Debugging and Understanding}
Given a crash online, our simulator can be used to try and replicate the environment 
before the crash to try and discover a trace violation. Given such a trace, we can diagnose what went wrong in the protocol implementation or the conceptual design.  

 


==> simulationold.tex <==
\section{Deterministic Simulation}
\label{sec:sim}
In this section, we describe our deterministic blockchain simulator. The goal of the deterministic blockchain simulator is to 
control uncertain parameters present in a real world blockchain and to allow us to capture the network-wide state from 
multiple node instances. 

Our simulator is designed so that the software component under test, in our case the consensus protocol, is agnostic to being run in a 
real client or simulated environment. To enable this, we mock other components and the network while exposing parameters such as 
delays, faults, etc. to be controlled via a simulator configuration containing user defined values for these parameters.  

Another feature of our simulator is the use of a Discrete-event simulation (DES). A discrete-event simulation (DES) models the operation of a system as a (discrete) sequence of events in time. Each event occurs at a particular instant in time and marks a change of state in the system. 
Between consecutive events, no change in the system is assumed to occur; thus the simulation time can directly jump to the occurrence time of the next event, which is called next-event time progression. The DES allows for faster testing, 
compared to using time intervals via the CPU clock. Instead of relying on chance, we can deliberately create a harsh simulated environment that quickly causes bugs in the protocol. 

Lastly, our simulator removes random behavior.  For instance, we avoid multi-threading, randomness, physical layers etc. Thus, we guarantee that every bug found can be reproduced and thus more easily diagnosed, and fixed. 


\begin{figure}
    \centering
    \includegraphics[width=0.60\linewidth]{figures/Simulator1.pdf}
    \caption{Deterministic Blockchain Simulator Simulator\label{fig:sim}}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.55\linewidth]{figures/Simulator2.pdf}
%    \caption{Simulated Consensus Protocol in Node}
%        \label{fig:node}
%\end{figure}

%    \begin{figure*}
%    \centering
%    \begin{subfigure}{0.30\textwidth}
%    \includegraphics[width=0.9\textwidth]{figures/Simulator1.pdf}
%    \caption{Deterministic Blockchain Simulator}
%    \label{fig:sim}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.33\textwidth}
%    \includegraphics[width=0.9\textwidth]{figures/Simulator2.pdf}
%    \caption{Simulated Consensus Protocol in Node}
%    \label{fig:node}
%    \end{subfigure}
%    \label{fig:tradvslive}
%    \end{figure*}


Figure~\ref{fig:sim} illustrates the structure of the deterministic 
simulator for testing a consensus protocol. The simulator contains several 
instances of the consensus protocol connected to other external components such 
as the mocked network and virtual clock. In the case of Workflow I, the user supplies ranges of parameters via the configuration file (config.) that the fuzzer component uses to generate synthetic workloads and inject faults. For Workflow II, a 
set of traces are provided as input. The simulator drives the nodes and network to operate (in virtual time) by following the actions in a given input trace. Because the actions in the trace (from the model) are not one-to-one with the 
actions of the simulated implementation, we implement a mapping between the actions as a table that is provided in the configuration file. The checker after an action is performed compares the resultant state with the state in the trace and makes sure they are compatible. Aside from producing traces for Workflow I, the simulator also 
measures several performance metrics that can be configured. These measurements are outputted in a metrics file and used for performance analysis as described in Section~\ref{sec:app}. We note that the deterministic simulator has been implemented such that the node (client code) does not have to be implemented in the same language as the simulator. 
